Risk-Averse Certification of Bayesian Neural Networks

In light of the inherently complex and dynamic nature of real-world environments, incorporating risk measures is crucial for the robustness evaluation of deep learning models. In this work, we propose a Risk-Averse Certification framework for Bayesian neural networks called RAC-BNN. Our method leverages sampling and optimisation to compute a sound approximation of the output set of a BNN, represented using a set of template polytopes. To enhance robustness evaluation, we integrate a coherent distortion risk measure--Conditional Value at Risk (CVaR)--into the certification framework, providing probabilistic guarantees based on empirical distributions obtained through sampling. We validate RAC-BNN on a range of regression and classification benchmarks and compare its performance with a state-of-the-art method. The results show that RAC-BNN effectively quantifies robustness under worst-performing risky scenarios, and achieves tighter certified bounds and higher efficiency in complex tasks.

==> Section/Main_result.tex <==
\section{Main Results}
In this section, we will develop a sampling-based solution to the probabilistic safety problem. 
According to the posterior distribution $\Prob{W}$ and the input distribution $\Prob{X}$, we can collect a group of  i.i.d. sampled inputs $x_i\in \mathbb{X}$ and a group of i.i.d. sampled parameters $w_j\in \mathbb{W}$. Using these samples, we compute the output samples $y_{ij}=f(x_i,w_j)$ and rewrite these  samples as $y_k$ for notation simplicity and let $N$ be the total number of samples.  

\subsection{Support Set Approximation}
Consider a convex template polytope  $\mathbb{P}$ in the form of 
\begin{eqnarray}\label{Eq:Pset}
\mathbb{P}=\{z\in \mathbb{R}^n\mid Vz\leq \bm{1}\}
\end{eqnarray}
where $V\in\mathbb{R}^{l\times n} $ and $L$ is the number of half spaces or inequalities.  
Given the set $\mathbb{P}$ in \eqref{Eq:Pset}, and $\bm{ \theta}\in \mathbb{R}^{L}$, let 
us introduce a parameterised set in the form of 
\begin{align}\label{Eq:Wva}
	\mathcal{H}(\bm{ \theta}):=	\{z\in \mathbb{R}^{n}\mid  V z\leq \bm{ \theta}\}.
\end{align} 




 Then, we approximate the output set $\mathbb{Y}$ by computing the optimal  parameterised set $\mathcal{H}(\bm{ \theta}_N^\star)$, where  $\bm{ \theta}_N^\star$ is the optimal solution to following optimisation problem 
\begin{eqnarray}\label{Opt:quanset}
	\begin{cases}
		&\min\limits_{\bm{\theta}}\quad  \bm{1}^T  \bm{\theta}    \\
		& \hspace{0.1cm}{\text s.t}:
		\begin{cases}
			Vy_k \leq \bm{ \theta} , k=1,\cdots,N, \\
			\bm{ \theta} \in \mathbb{R}^L.
		\end{cases}
	\end{cases}
\end{eqnarray}  
% \zf{Do we need to add  regularizer?}

\begin{proposition}\label{Prop: risk bound}
	The optimal solution $\bm{ \theta}_N^\star$ to \eqref{Opt:quanset} is  
\begin{eqnarray}  
	[\bm{ \theta}_N^\star]_i=\max_{k=1,\cdots,N} [V]_i y_k,
\end{eqnarray}  
	where $[V]_i$ denotes $i$-th row of $V$.  
Let $\hat{\mathbb{Y}}_N=\mathcal{H}(\bm{ \theta}_N^\star)$.  Given   $\epsilon_1\in (0,1)$,  $\beta_1\in (0,1)$, and the Euler's constant $\text{e}$, if
	\begin{eqnarray} \label{Eq:samplenum} 
	N\geq \frac{1}{\epsilon_1} \frac{\text{e}}{\text{e}-1} \Bigl(\ln\frac{1}{\beta_1} + n+L \Bigr),
	\end{eqnarray}  
	then, with probability no less than $1-\beta_1$, 
	\begin{eqnarray}  \label{Eq:errorbound}
	\mathbb{P}[y\in \mathbb{Y}: y\notin \hat{\mathbb{Y}}_N] =	\int_ {\mathbb{Y} }1_{\hat{\mathbb{Y}}_N^c}(\xi)\Prob{Y}(d \xi)
 \leq  \epsilon_1.
	\end{eqnarray}  
\end{proposition}

Proposition~\ref{Prop: risk bound}  provides a statistical gap between $\hat{\mathbb{Y}}$ and the true output set $\mathbb{Y}$.

\subsection{Evaluation of Output Distribution}

Given the output samples $\{y_k\}^N_{k=1}$, we denote the corresponding empirical distribution as $$\empProb{Y}{N}(y) = \frac{1}{N} \sum_{i = 1}^N \dirac{y_i} (y).$$


Consider the true output set $\mathbb{Y}$, the approximate set $\hat{\mathbb{Y}}_N$, and the true output distribution $\Prob{Y}$. 
When $\mathbb{Y} \nsubseteq \hat{\mathbb{Y}}_N$, let us define an approximate output distribution $\bar{\Prob{Y}}$ supported onto  $\hat{\mathbb{Y}}_N$: 
\begin{equation}
\bar{\Prob{Y}}(y)=\begin{cases}
	\Prob{Y}(y), \text{ if } y\in \mathbb{Y}\cap \hat{\mathbb{Y}}_N, \\
	\frac{1-\int_{\hat{\mathbb{Y}}_N\cap\mathbb{Y}}\Prob{Y}(d \xi)}{{\text Leb}(\hat{\mathbb{Y}}_N\setminus \mathbb{Y})}, \text{ otherwise},
\end{cases}
\end{equation}
where ${\text Leb}$ denotes the Lebesgue measure. 



\begin{proposition}\label{Pro:evadis}
Given $\beta_2\in (0,1)$ and $N\in \mathbb{N}_{\geq 1}$, there exist $\epsilon_2$ and $\epsilon_3$ such that with  probability no less than $1-\beta_2$,  
	\begin{eqnarray}  
		&&  d^{\mathbb{Y}}_{\text W}(\Prob{Y},\empProb{Y}{N})\leq \epsilon_2, \\
		&&d^{\hat{\mathbb{Y}}_N}_{\text W}(\bar{\Prob{Y}},\empProb{Y}{N})\leq \epsilon_3.
		\end{eqnarray}  
\end{proposition}
{\color{blue}$\epsilon_2$: see Section 6.2.1.1 and Theorem 6.1 in \cite{rahimian2019distributionally} and Theorem 2 in \cite{fournier2015rate}. }




\subsection{Distributional Robust Evaluation}
Recall the set $\hat{\mathbb{Y}}_N=\{z\in \mathbb{R}^n\mid Vz\leq \bm{\theta}^*\}$, where $V\in \mathbb{R}^{L\times n}$.
\begin{assumption}\label{Ass:SafesetS}
We assume that 
\begin{itemize}
    \item[(A1)] the  function $h:\Rb^n \mapsto \Rb$ is  proper, concave, and lower semi-continuous; 
    \item[(A2)] $h$ is Lipschitz continuous with respect to a constant $L\geq 0$;
    \item[(A3)]  there exists a finite $h_{\max}> 0$ such that  $|h(y)|\leq h_{\max}$, $\forall y\in \mathbb{Y}$.
\end{itemize}
\end{assumption}

\begin{proposition}
    Suppose the assumption A1 holds. Then,
    With probability no less than $1-\beta_2$, 
    \begin{eqnarray}  
Perf	\leq  \sup_{\Prob{Y}'\in \mathbb{B}_{\epsilon_2}(\empProb{Y}{N})}\int_{\Rb^\outdim} h(\xi)\Prob{Y}'(d \xi) = \frac{1}{N}\sum_{k=1}^N h(\xi_k^*).
\end{eqnarray}  
where the ambiguity set $\mathbb{B}_{\epsilon_2}(\empProb{Y}{N})=\{\Prob{Y}' \mid d^{\Rb^\outdim}_{\text W}(\Prob{Y}',\empProb{Y}{N})\leq \epsilon_2 \}$, $\xi_k^*= y_k - q_k^*$, and 
$q_i^*$ is the value of $q_i$ that attains the supremum of the following finite convex program
\begin{align}
    \sup_{q_k} \quad  &\frac{1}{N}\sum_{k=1}^N h(y_k - q_k) \nonumber \\
    s.t. \quad & \frac{1}{N} \sum_{k=1}^N \left\| q_k\right\| \leq \epsilon_2.
\end{align}

\end{proposition}

\begin{theorem}
Suppose that the assumptions A1--A3 hold. Let $\zeta=2 h_{\max} \epsilon_1 +L \epsilon_2+L \epsilon_3$. With probability no less than $1-\max\{\beta_1,\beta_2\}$,  
  \begin{align}
Perf	&\leq  \sup_{\Prob{Y}'\in \mathbb{B}_{\epsilon_3}(\empProb{Y}{N})}\int_{\hat{\mathbb{Y}}_N} h(\xi)\Prob{Y}'(d \xi) + \zeta \\
&= \frac{1}{N}\sum_{k=1}^N h(\xi_k^*)+\zeta. 
  \end{align}  
where the ambiguity set $\mathbb{B}_{\epsilon_3}(\empProb{Y}{N})=\{\Prob{Y}' \mid d^{\hat{\mathbb{Y}}_N}_{\text W}(\Prob{Y}',\empProb{Y}{N})\leq \epsilon_3 \}$, $\xi_k^*= y_k - q_k^*$, and 
$q_k^*$ is the value of $q_k$ that attains the supremum of the following finite convex program
\begin{align}
       \sup_{q_k} \quad  &\frac{1}{N}\sum_{k=1}^N h(y_k - q_k) \nonumber \\
    s.t. \quad & \frac{1}{N} \sum_{k=1}^N \left\| q_k\right\| \leq \epsilon_3 \nonumber \\
    &y_k -q_k \in  \hat{\mathbb{Y}}_N, \forall k \leq N.
\end{align}
\end{theorem}

{\color{blue}
\begin{assumption}
The function $h(\xi)$ is convex.
\end{assumption}

\begin{theorem}
Suppose that the assumptions A2, A3, 2 hold. With probability no less than $1- \max\{\beta_1,\beta_2\}$,
\begin{align}
Perf	&\geq  \inf_{\Prob{Y}'\in \mathbb{B}_{\epsilon_3}(\empProb{Y}{N})}\int_{\hat{\mathbb{Y}}_N} h(\xi)\Prob{Y}'(d \xi) + \zeta \\
&= \frac{1}{N}\sum_{k=1}^N h(\underline{\xi}_k^*)+\zeta. 
\end{align} 
where $\underline{\xi}_k^*= y_k - \underline{q}_k^*$, and 
$\underline{q}_k^*$ is the value of $q_k$ that attains the supremum of the following finite convex program
\begin{align}
       \sup_{q_k} \quad  &\frac{1}{N}\sum_{k=1}^N -h(y_k - q_k) \nonumber \\
    s.t. \quad & \frac{1}{N} \sum_{k=1}^N \left\| q_k\right\| \leq \epsilon_3 \nonumber \\
    &y_k -q_k \in  \hat{\mathbb{Y}}_N, \forall k \leq N.
\end{align}
\end{theorem}


}
{\color{blue}
\subsection{BNN}
Consider $h(\xi) = \max_{i\leq I} \langle a_i,\xi\rangle + b_i$.
}

% Suppose that Assumption A1 holds. Then, the strong duality can be further writen as 
% \begin{align}
%     \inf_{\beta,s_i,z_{i},v_i} & \beta \epsilon_3 + \frac{1}{N}\sum_{i=1}^N s_i \\
%     s.t. \quad  &[-l]^{*}(z_i - v_i) +\sigma_{ \hat{\mathbb{Y}}_N}(v_i) - \langle z_i, \hat{\xi}_i \rangle, \forall i \leq N \\
%     &\left\| z_i\right\|_{*} \leq \beta, \forall i\leq N.
% \end{align}
% where $[-l]^{*}(z_i - v_i)$ denotes the conjugate of $-l$ evaluated at $z_i - v_i$, $\left\|z_i\right\|_{*}$ is the dual norm of $z_i$, and $\sigma_{ \hat{\mathbb{Y}}_N}$ is the support function of $\hat{\mathbb{Y}}_N$.


\section*{Appendix}
\begin{lemma}\label{Eq:LCWd}
Suppose that the function $h:\Rb^n \mapsto \Rb$ is Lipschitz continuous with respect to a constant $L\geq 0$. For any two probability distribution $\Prob{Y}, \Prob{Y}' \in \mathcal{P}(\mathbb{Y})$, 
\begin{align}
    | \int_{\mathbb{Y}} h(\xi)\Prob{Y}(d \xi)-  \int_{\mathbb{Y}} h(\xi) \Prob{Y}'(d \xi)| \leq L d^{\mathbb{Y}}_{\text W}(\Prob{Y},\Prob{Y}'). 
\end{align}
\end{lemma}
\textbf{Proof of Theorem 2}. 
    Recall that $Perf= \int_{\mathbb{Y}}  h(\xi) \Prob{Y}(d\xi)$. We have that 
\begin{align}\label{eq:thm2:1}
   & | \int_{\mathbb{Y}} h(\xi)\Prob{Y}(d \xi)-  \int_{\hat{\mathbb{Y}}_N} h(\xi)\bar{\Prob{Y}}(d \xi)| \nonumber\\
   =&| \int_{\mathbb{Y}} h(\xi)\Prob{Y}(d \xi)- \int_{\hat{\mathbb{Y}}_N} h(\xi)\Prob{Y}(d \xi) \nonumber  \\
   & +\int_{\hat{\mathbb{Y}}_N} h(\xi)\Prob{Y}(d \xi) -\int_{\hat{\mathbb{Y}}_N} h(\xi)\empProb{Y}{N}(d \xi) \nonumber \\ 
   & +\int_{\hat{\mathbb{Y}}_N} h(\xi)\empProb{Y}{N}(d \xi)-\int_{\hat{\mathbb{Y}}_N} h(\xi)\bar{\Prob{Y}}(d \xi)| \nonumber \\
   \leq  &| \int_{\mathbb{Y}} h(\xi)\Prob{Y}(d \xi)- \int_{\hat{\mathbb{Y}}_N} h(\xi)\Prob{Y}(d \xi)| \nonumber  \\
   & +|\int_{\hat{\mathbb{Y}}_N} h(\xi)\Prob{Y}(d \xi) -\int_{\hat{\mathbb{Y}}_N} h(\xi)\empProb{Y}{N}(d \xi)| \nonumber \\ 
   & +|\int_{\hat{\mathbb{Y}}_N} h(\xi)\empProb{Y}{N}(d \xi)-\int_{\hat{\mathbb{Y}}_N} h(\xi)\bar{\Prob{Y}}(d \xi)|.
\end{align}  

For the first item, it follows from the boundedness of $h(y)$ over $\mathbb{Y}$ and   Proposition~\ref{Prop: risk bound} that   with probability no less than $1-\beta_1$, 
\begin{align} \label{eq:thm2:2}
| \int_{\mathbb{Y}} h(\xi)\Prob{Y}(d \xi)- \int_{\hat{\mathbb{Y}}_N} h(\xi)\Prob{Y}(d \xi)| \leq h_{\max} \epsilon_1. 
\end{align}  

Let us address the second item. 
According to Lemma~\ref{Eq:LCWd},  Proposition~\ref{Pro:evadis}, and  \eqref{eq:thm2:2}, it follows that   with probability no less than $1-\max\{\beta_1,\beta_2\}$,   
\begin{align}  \label{eq:thm2:3}
&|\int_{\hat{\mathbb{Y}}_N} h(\xi)\Prob{Y}(d \xi) -\int_{\hat{\mathbb{Y}}_N} h(\xi)\empProb{Y}{N}(d \xi)| \nonumber \\
=& |\int_{ \mathbb{Y}} h(\xi)\Prob{Y}(d \xi)  -\int_{\mathbb{Y}} h(\xi)\empProb{Y}{N}(d \xi)-\int_{\hat{\mathbb{Y}\setminus (\mathbb{Y}}_N \cap \mathbb{Y})} h(\xi)\Prob{Y}(d \xi)|  \nonumber \\
\leq & |\int_{ \mathbb{Y}} h(\xi)\Prob{Y}(d \xi)  -\int_{\mathbb{Y}} h(\xi)\empProb{Y}{N}(d \xi)|+|\int_{\hat{\mathbb{Y}\setminus (\mathbb{Y}}_N \cap \mathbb{Y})} h(\xi)\Prob{Y}(d \xi)| \nonumber \\
\leq & L \epsilon_2 + \leq h_{\max} \epsilon_1.  
\end{align} 

Similarly, we can address the third item by concluding that with probability no less than $1-\beta_2$,  
\begin{align}  \label{eq:thm2:4}
|\int_{\hat{\mathbb{Y}}_N} h(\xi)\empProb{Y}{N}(d \xi)-\int_{\hat{\mathbb{Y}}_N} h(\xi)\bar{\Prob{Y}}(d \xi)|  \leq L \epsilon_3.
\end{align}  
Combining \eqref{eq:thm2:1}--\eqref{eq:thm2:4}, we have
\begin{align}
   & | \int_{\mathbb{Y}} h(\xi)\Prob{Y}(d \xi)-  \int_{\hat{\mathbb{Y}}_N} h(\xi)\bar{\Prob{Y}}(d \xi)| \nonumber \\
   \leq & 2 h_{\max} \epsilon_1 +L \epsilon_2+L \epsilon_3 :=\zeta.
\end{align}  
% Thus, we conclude that 
% Following Propositions~\ref{Prop: risk bound}--\ref{Pro:evadis}, 
Thus, we have that with probability no less than $1-\max\{\beta_1,\beta_2\}$, 
\begin{align}
     Perf &\leq \int_{\hat{\mathbb{Y}}_N} h(\xi)\bar{\Prob{Y}}(d \xi) + \zeta \nonumber \\
     &\leq \sup_{\Prob{Y}'\in \mathbb{B}_{\epsilon_3}(\empProb{Y}{N})}\int_{\hat{\mathbb{Y}}_N} h(\xi)\Prob{Y}'(d \xi) + \zeta,
\end{align}
% and {\color{red}
% \begin{align}
%      Perf &\geq \int_{\hat{\mathbb{Y}}_N} h(\xi)\bar{\Prob{Y}}(d \xi) - \zeta \nonumber \\
%      &\geq \inf_{\Prob{Y}'\in \mathbb{B}_{\epsilon_3}(\empProb{Y}{N})}\int_{\hat{\mathbb{Y}}_N} h(\xi)\Prob{Y}'(d \xi) - \zeta,
% \end{align}}
where the ambiguity set $\mathbb{B}_{\epsilon_3}(\empProb{Y}{N})=\{\Prob{Y}' \mid d^{\hat{\mathbb{Y}}_N}_{\text W}(\Prob{Y}',\empProb{Y}{N})\leq \epsilon_3 \}$. 
%\begin{proof}
 %   \begin{eqnarray}  
%		| \int_ {\mathbb{S} \cap\mathbb{Y}}{\text Pr}^y(dy)-  \int_ {\mathbb{S} \cap\hat{\mathbb{Y}}}\bar{\text Pr}^y(dy)| \leq \underbrace{\epsilon_1 + 2\epsilon_2}_{:=\zeta}.
%	\end{eqnarray}  
%\end{proof}


% \textcolor{blue}{
% Strong duality: \cite{esfahani2015data}
% \begin{align}
%     &\sup_{\Prob{Y}'\in \mathbb{B}_{\epsilon_3}(\empProb{Y}{N})}\int_{\hat{\mathbb{Y}}_N} h(\xi)\Prob{Y}'(d \xi) \nonumber \\
%     &= \inf_{\beta\geq 0}\{ \frac{1}{N} \sum_{i=1}^N \max_{\xi \in \empProb{Y}{N}} \{ h(\xi) -\beta \| \xi - y_i\|  \} + \epsilon_3 \beta \}
% \end{align}
% According to \cite{esfahani2015data}, the worst case distribution is characterized by 
% $$
% Q^* = \frac{1}{N}\sum_{i=1}^N \delta_{\xi_{i}^*} \; with \; \xi_i^*: = \hat{\xi}_i - q_i^*,
% $$
% where $q_i^*$ is the value of $q_i$ that attains the supremum of the following finite convex program
% \begin{align}
%     \sup_{q_i} \quad  &\frac{1}{N}\sum_{i=1}^N l(\hat{\xi}_i - q_i) \nonumber \\
%     s.t. \quad & \frac{1}{N} \sum_{i=1}^N \left\| q_i\right\| \leq \epsilon_3 \nonumber \\
%     &\hat{\xi}_i -q_i \in  \hat{\mathbb{Y}}_N, \forall i \leq N.
% \end{align}
% Then, 
% \begin{align}
%     \sup_{\Prob{Y}'\in \mathbb{B}_{\epsilon_3}(\empProb{Y}{N})}\int_{\hat{\mathbb{Y}}_N} h(\xi)\Prob{Y}'(d \xi) = \mathbb{E}_{Q_*}[h(\xi)] = \frac{1}{N}\sum_{i=1}^N l(\xi_i^*).
% \end{align}}


==> Section/Old_Problem_formulation.tex <==
\section{Preliminaries and Problem Formuation}
\label{sec:problem-statement}

In this section we introduce the necessary background and notations that will be employed throughout the paper.

\subsection{Notation}

Let $\mathcal{X} = \Rb^\indim$ and $\mathcal{Y} = \Rb^\outdim$ be the input and output space, respectively, and let $\mathcal{\paramSet} = \Rb^\paramdim$ be the parameter space. We denote by $\mathcal{P}(\mathcal{X})$ the set of probability distribution over $\mathcal{X}$, that is,
\begin{equation}
    \mathcal{P}(\mathcal{X}) = \left\{ \Prob{X}: \int_\mathcal{X} \Prob{X}(d\xi) = 1, \Prob{X} \geq 0 \right\},
    \label{eq:set-prob}
\end{equation}
similarly for $\mathcal{Y}$ and $\mathcal{W}$. Throughout the paper, the Euclidean spaces are equipped with their corresponding Borel $\sigma$-algebra and all measures are defined with respect it. More details can be found in \refhere. For a finite collection of points $\{x_1, \ldots, x_N\}$ in $\mathbb{X}$, we denote the corresponding empirical distribution as
\begin{equation}
    \empProb{X}{N}(x) = \frac{1}{N} \sum_{i = 1}^N \dirac{x_i} (x),
    \label{eq:emp-prob}
\end{equation}
similar for points in the output space $\mathcal{Y}$ and parameter space $\mathcal{\paramSet}$, where the empirial distribution will be denoted by $\empProb{Y}{N}$ and $\empProb{\paramSet}{N}$, respectively. Given two probability measures $\Prob{X}$ and $\Prob{X}'$ defined in the same space, i.e., $\Prob{X}, \Prob{X}' \in \mathcal{P}(\mathcal{X})$, we denote by $d_W(\Prob{X},\Prob{X}')$ the Kantorovich metric between these measures, defined as
\begin{equation}
    d^{\mathcal{X}}_W(\Prob{X},\Prob{X}') = \inf_{\pi \in \Pi(\Prob{X},\Prob{X}')} \int_{\mathcal{X}\times \mathcal{X}} \| \xi_1 - \xi_2 \| \pi(d \xi_1, d \xi_2),
    \label{eq:Kant-metric}
\end{equation}
where $\Pi(\Prob{X}, \Prob{X}')$ is the set of couplings (or joint distributions) with marginals given by $\Prob{X}$ and $\Prob{X}'$.


\subsection{Scenario Approach Theory}

A key feature of our technique is the use of the scenario optimization \refhere to obtain our sample complexity guarantees. We briefly describe the necessary result here for completeness and we refer the reader to the literature for a thorough introduction to the subject. Let $(\Omega, \mathcal{F}, \mathbb{P})$ be a general probiblity measure space, where $\Omega$ is the uncertainty set, $\mathcal{F}$ is a $\sigma$-algebra, and $\mathbb{P}$ is a probability measure defined on $\mathcal{F}$. The scenario optimization allows us to generate a feasible solution to the chance-constrained optimization problem given by
\begin{equation}
    \begin{aligned}
        \minimize_x & \quad c^\top x \\ 
        \subjecto & \quad \mathbb{P}\{ \omega \in \Omega: g(x,\eta(\omega)) \leq 0\} \geq 1-\epsilon,
    \end{aligned}
    \label{eq:chance-constrained}
\end{equation}
where $\epsilon \in (0,1)$, $g: \Rb^d \times \Rb^q \mapsto \Rb$ is a convex function in the first argument and measurable in the second one, and $\eta:\Omega \mapsto \Rb^q$ is a random variable defined on $\Omega$ with values on $\Rb^q$. In fact, the \refhere show the following bound on the probability of constraint associated with the optimal solution of optimization problem
%
\begin{equation}
    \begin{aligned}
        \minimize_x & \quad c^\top x \\
        \subjecto & \quad g(x,\eta(\omega)) \leq 0, \text{ for all } \omega \in \mathcal{D},
    \end{aligned}
    \label{eq:scenario-program}
\end{equation} 
%
where $\mathcal{D} = \{\omega_1,\ldots,\omega_N\}$ is the collection of i.i.d. samples from the random variable $\eta$.
\begin{theorem}[\refhere]
    Assume that the optimal solution of \eqref{eq:scenario-program} exists and is unique, and that the interior of the feasible set of \eqref{eq:scenario-program} is non-empty, both almost surely with respect to the measure on the samples in $\mathcal{D}$. Then we have that
    \begin{align*}
        \mathbb{P}^N\{\mathcal{D} \in \Omega^N: \mathbb{P}\{\omega \in \Omega: g(x^\star(D),\omega) > 0 \}  > \epsilon \} \\ \leq \sum_{i = 0}^{d-1} {N \choose i} \epsilon^i (1-\epsilon)^{d-i},
        \label{eq:scenario-program-theo}
    \end{align*}
    where $d$ is the dimension of the vector $x$ in \eqref{eq:scenario-program}, and $x^\star(\mathcal{D}): \Omega \mapsto \Rb^d$ is the unique solution of \eqref{eq:scenario-program}.
    \label{theo:scenario-optimization}
\end{theorem}

The bound of Theorem \ref{theo:scenario-optimization} can not be improved, as it holds with equality for the class of fully-supported optimization problems (see \refhere for more details). In the following section, we will invoke Theorem \ref{theo:scenario-optimization} to assert properties of the output distribution of a BNN.


\subsection{Bayesian Neural Network}

In this section, we first review the concepts of Bayesian neural networks (BNNs) using the notation introduced in the previous section. 


\begin{definition}[Bayesian Neural Networks] A pair $(f, \Prob{W})$, where $f:\mathcal{X} \times \mathcal{W} \mapsto \mathcal{Y}$ is a continuous function and $\Prob{W} \in \mathcal{P}(\mathcal{W})$ is a measure in the parameter space $\mathcal{W}$, is called a Bayesian Neural Network (BNN).
   \label{defi:BNN} 
\end{definition}


Starting with a prior distribution  $p(w)$, we can infer network parameters to compute the posterior distribution $p(w|\dataset)$ of parameters conditioned on dataset $\dataset= \{(x_i, y_i)\in \mathcal{X}\times \mathcal{Y}: i = 1, \ldots, N\}$. 
With dataset $\dataset$ observed, the prior distribution of a BNN is updated according to the likelihood, $p(\dataset | w) = \prod_{i=1}^{n_\dataset} p(y_i | x_i, w)$, which models how likely the outputs are observed under the stochasticity of model parameters and observational noise.
The posterior distribution, given the dataset, is then computed by means of the Bayes formula, i.e., $p(w | \dataset) \propto p(\dataset | w) p(w)$. 
In practice, the posterior distribution $p(w | \dataset)$ can be obtained by  different 
inference techniques, e.g., Hamiltonian Monte Carlo (HMC)\refhere, Variational Inference (VI)\refhere, and Monte Carlo Dropout (MCD) \refhere. 
 Note that  the measure $\Prob{W} \in \mathcal{P}(\mathcal{W})$ in Definition~\ref{defi:BNN}  refers to  the  posterior distribution $p(w | \dataset)$.

%The posterior $p(w | \dataset)$ then induces the distribution over outputs called the posterior predictive distribution for an input point $x^*$, which is defined as: 
%\begin{equation}\label{eq:pred_distr}
%    p(y^* | x^*, \mathcal{D}) = \int p(y^{*} | x^{*}, w)p(w | \mathcal{D}) dw.
%\end{equation}


 %\textbf{Langevin Dynamics:} the taget distribution is a stationary distribution associated with an stochastic differential equation (SDE). Samples are obtained by propagating the SDE forward (or backward) in time.






%The final decision is obtained using Bayesian decision theory, which selects the value $\hat{y}$ that minimises the Bayesian risk of an incorrect prediction according to the posterior predictive distribution and the loss function $\mathcal{L}$:
%\begin{align*}
%\hat{y} = \argmin_{y} \int_{\outset} \mathcal{L}(y, y^*) p(y^* | x^*, \dataset) dy^*.
%\end{align*}
% which 
%For classification (0-1 loss), this corresponds to selecting the class that maximises the predictive distribution:
%\begin{align}\label{eq:bnn_decision}
%    \hat{y} = \argmax_{i=1,\ldots,m} p_i(y^* | x^*, \mathcal{D}) = \argmax_{i=1,\ldots,m} \mathbb{E}_{w \sim \post}\left[ \sigma_i(f^w(x)) \right]
%\end{align}
%where $\sigma_i$ indicates the $i$-th component of the softmax function.



\subsection{Problem Statement}

Our goal is to study the probabilistic safety problem of BNN. 



\begin{problem}[Probabilistic safety for BNNs]\label{Prob:SafeBNN}
Consider a BNN $(f,\Prob{W})$.  Let $\mathbb{X}\subset \mathcal{X}$ be a compact set of input,  $\Prob{X} \in \mathcal{P}(X)$ be a measure with support included in $\mathbb{X}$. Given a performance function $h: \Rb^n \mapsto \Rb$, evaluate  the upper bound of the expected loss 
\begin{equation} \label{eq:loss}
 Perf= \int_{\mathbb{X}}  \int_{\mathcal{W}} h(f(\xi_2,\xi_1))\Prob{\paramSet}(d\xi_1)\Prob{X}(d\xi_2).
\end{equation}
%For a given $\epsilon \in (0,1)$, verify if a given set  $\mathbb{S} \subset \mathcal{Y}$ is a probabilistic safe with a level $\epsilon$, that is,    
%\begin{equation} \label{eq:prob-safety-level}
% p_{\text safe}(\mathbb{S})=:  \int_{\mathcal{X}}  \int_{\mathcal{W}} (1_{\mathbb{S}} \circ f)(x,\xi_1) \Prob{\paramSet}(d\xi_1)\Prob{X}(d\xi_2) \geq 1-\epsilon.
%\end{equation}
\end{problem}

Due to the complex architecture of BNNs, exact computation of the integral in \eqref{eq:loss} is intractable.    An alternative solution to solve Problem~\ref{Prob:SafeBNN} is to consider the following two subproblems: (1) support evaluation problem, that is, characterize the output set $\mathbb{Y}=\{f(x,w) \mid x\in\mathbb{X},w\in\mathcal{W}\}$; and (2) distribution evaluation problem, that is, given the input distribution $\Prob{X}$ and the parameter distribution $\Prob{W}$,  characterize output distribution  $\Prob{Y}$. Then, we can rewrite \eqref{eq:loss}  as 
\begin{equation} \label{eq:loss1}
 Perf= \int_{\mathbb{Y}}  h(\xi) \Prob{Y}(d\xi).
\end{equation}

Since the map $f$ of the BNN is nonlinear, exact computation of $\mathbb{Y}$ is hard (except that the set $\mathbb{Y}=\mathbb{R}^n$).  In our work, we aim at developing a new sampling-based algorithm to approximate the set $\mathbb{Y}$ with polynomial computational complexity and statistical guarantees.   
Evaluation of $\Prob{Y}$ is also intractable. Leveraging the sampling-based method, we will characterize a Wasserstein
ambiguity set, i.e., a ball of probability distributions defined
using the Wasserstein distance, that contains $\Prob{Y}$ with high confidence.  




%More specifically, we can guarantee that the  statistical gap between the approximated set $\hat{\mathbb{Y}}$ and the  convex hull of the true reachable set ${\text Conhull}(\mathbb{Y})$ 

==> Tables/RQ_Comparison.tex <==
\begin{table}[h]
\caption{Comparison with BNN-DP in certification bounds and computation time}
    \label{tab:comparison}
    \centering
      \footnotesize	
    \begin{tabular}{ccccccccc}
        \toprule
        \multirow{2}{*}{\textbf{Method}} & \multicolumn{2}{c}{2D Noisy Sine} & \multicolumn{2}{c}{2D Noisy Sine} & \multicolumn{2}{c}{Kin8nm} & \multicolumn{2}{c}{MNIST}\\
        \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9}
        & $\gamma$-robustness & Time (s)  & $\gamma$-robustness & Time (s)  &$\gamma$-robustness & Time (s)  &$\gamma$-robustness & Time (s)\\
        \midrule
        BNN-DP & 0.065 & 6.148 & 2.042 & 8.371 & 0.137 & 7.886 \\
        BNN-Cert\_0.1 & 0.1 & \textbf{0.815} & 0.1 & \textbf{0.757} & 0.1 & \textbf{0.984} & & \\
        BNN-Cert\_0.05 & \textbf{0.05} & 1.640 & \textbf{0.05} & 1.761 & \textbf{0.05} & 1.893 & &\\
        \bottomrule
    \end{tabular}
    
\end{table}
